SeFoRA: Sketch-Aggregated Federated Low-Rank Adaptation with Heterogeneous Client Ranks

We consider federated parameter-efficient fine-tuning of foundation models, e.g., LLMs and LVMs, using low-rank adaptation (LoRA; ~Hu et al.\ 2022). Combining LoRA with federated learning introduces challenges absent from either setting alone: clients may use different LoRA ranks, making their factor matrices dimension-incompatible, and factor-wise averaging suffers from a bilinear mismatch. We propose SeFoRA, a sketch-aggregated federated LoRA algorithm in which each client transmits a linear sketch of its local $\Delta \mathbf{W}$ updates, enabling direct aggregation at the federator. As a result, SeFoRA overcomes the rank heterogeneity challenge and alleviates the bilinear mismatch. We establish convergence to a neighborhood of a first-order stationary point at rate $\\mathcal{O}(T^{-1/2})$. Extensive numerical experiments on language and vision models showcase the performance of our algorithm compared to existing methods.

==> macros.tex <==
\newcommand{\Loss}{\mathcal{L}}
\newcommand{\Dataset}{\mathcal{D}}

\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
    \let\mathaccent\save@mathaccent
    \if#32 \let\macc@nucleus\first@char \fi
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
    \ifdim\dimen@>\z@ \dimen@0pt\fi
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother


\newcommand{\cO}{\mathcal{O}}
\newcommand{\model}{\mathbf{W}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\B}{\mathbf{B}}

\newcommand{\Bh}{\widehat{\B}}
\newcommand{\Ah}{\widehat{\A}}

\newcommand{\Update}{\Delta \mathbf{W}}
\newcommand{\Updatebar}{\widebar{\Update}}
\newcommand{\mOme}{\mathbf{\Omega}}
\newcommand{\mPsi}{\mathbf{\Psi}}
\newcommand{\Trunc}{\mathbf{\Gamma}}
\newcommand{\TupleA}{\mathbf{\mathtt{A}}}
\newcommand{\TupleB}{\mathbf{\mathtt{B}}}
\newcommand{\TupleY}{\mathbf{\mathtt{Y}}}
\newcommand{\TupleZ}{\mathbf{\mathtt{Z}}}
\newcommand{\TupleModel}{\mathbf{\mathtt{W}}}
\newcommand{\TupleUpdate}{\Delta \mathbf{\mathtt{W}}}
\newcommand{\TupleUpdatebar}{\widebar{\TupleUpdate}}
\newcommand{\TupleTrunc}{\mathbf{\mathtt{\Gamma}}}

\newcommand{\TruncOpe}{\mathfrak{\Gamma}}

\newcommand{\U}{\mathbf{{U}}}
\newcommand{\V}{\mathbf{{V}}}
\newcommand{\bSigma}{\mathbf{{\Sigma}}}

\DeclareMathOperator{\argmin}{\mathrm{argmin}}
\DeclareMathOperator{\rank}{\mathrm{rank}}



\newcommand{\defeq}{\ensuremath{\triangleq}}

\newcommand{\WeightDecay}{\lambda}



\newcommand{\yx}[1]{\textcolor{orange}{\footnotesize[#1-yue]}}
\usepackage{longfbox}
\newcommand{\mb}[1]{~{\textcolor{gray!50!purple}{\textbf{[}#1 -- \small M\textbf{]}}}}
\newtheorem{assumption}{Assumption}
\crefname{assumption}{Assumption}{Assumptions}

\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{corollary}{Corollary}



\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
\newcommand{\rb}[1]{\textcolor{bleudefrance}{\footnotesize [#1 -- rawad]}}
\newcommand{\tj}[1]{\textcolor{magenta}{\footnotesize [#1 -- tayyebeh]}}



\newcommand{\cmark}{\ensuremath{\checkmark}}
\newcommand{\xmark}{\ensuremath{\times}}
\newcommand{\hetalgname}{\texttt{\textsc{SeFoRA}}\xspace}

